Transient Nonlinear Electrothermal Adjoint Sensitivity Analysis for HVDC Cable Joints

Efficient computation of sensitivities is a promising approach for efficiently of designing and optimizing high voltage direct current cable joints. This paper presents the adjoint variable method for coupled nonlinear transient electrothermal problems as an efficient approach to compute sensitivities with respect to a large number of design parameters. The method is used to compute material sensitivities of a 320kV high voltage direct current cable joint specimen. The results are validated against sensitivities obtained via the direct sensitivity method.

==> cable_joint_specimen.tex <==
 \label{ch:joint_specimen}
 \begin{figure}[tb]%
	\centering
	\includegraphics[width=0.6\columnwidth]{figs/model_6.pdf}
\vspace{0.2cm}
\caption{\begingroup \small Schematic of the investigated \ac{hvdc} cable joint \cite{Hussain_2017aa} in a cylindrical coordinate system $(\varrho,z)$. The numbers indicate the different materials as described in the text, the \ac{fgm} layer is highlighted in green. The red line marks the interface between the \ac{fgm} layer and the cable insulation. The cable joint is surrounded by a 30\,cm thick layer of sand and buried 2\,m beneath the ground. 
\endgroup}\label{Muffe Konfiguration}
\end{figure}

Figure~~\ref{Muffe Konfiguration} shows a cut of the investigated 320\,kV \ac{hvdc} cable joint model \cite{Hussain_2017aa}. 
The cable joint connects two cables segments, each consisting of a copper conductor (domain 1), an insulation layer (domain 4) and a grounded outer sheath (domain 8). The conductors are connected by an aluminum connector (domain 2), which is encased in conductive \ac{sir} (domain 3). The primary insulation of the cable (domain 4) is composed of \ac{xlpe}, while the main insulation of the cable joint body (domain 5) is made from insulating \ac{sir}. The outer sheath of the cable joint (domain 7) as well as the outer semiconductor of the cable (domain 8) are grounded. %To implement resistive field grading, 
The cable joint is surrounded by a 30\,cm thick layer of sand and buried 2\,m beneath the ground. 

In the simulation, a switching impulse overvoltage is applied to the domains 1 to 3, which are modeled as \acp{pec} due to their substantially higher conductivities relative to the insulating materials. 
The assumed operating temperatures are 65$^\circ$C at the copper conductors and 20$^\circ$C for the ambient temperature at the top of the soil layer \cite{Spack_2021ab}. For a detailed description of the geometric measurements of the cable joint and material characteristics, see \cite{Spack_2021ab, Hussain_2017aa}.
%(\clr{ToDo: Specify; Check values in COMSOL)}.

To mitigate harmful electric field stresses at the insulation interfaces between the \ac{xlpe} and \ac{sir}, a layer of nonlinear \ac{fgm} (domain 6) is introduced. This \ac{fgm} layer dynamically adjusts its conductivity based on the local electric field strength, $E$. In regions of high electric field stress, the \ac{fgm}'s conductivity increases, thereby redistributing the electric field by shifting the voltage drop to less stressed areas. This results in a more balanced electric field distribution across the insulation layers. 

The nonlinear conductivity of the \ac{fgm}, $\sigma_{\+{FGM}}$, is modeled by the following function \cite{Hussain_2017aa}:
\begin{equation}\label{Conductivity}
\begin{split}
\sigma_{\+{FGM}}&(E,\theta)=p_{1}\frac{1+p_{4}^{(E-p_{2})p_{2}^{-1}}}{1+p_{4}^{(E-p_{3})p_{2}^{-1}}}\+{exp}(-p_{5}(\theta^{-1}-\theta_{0}^{-1}))\,,
\end{split}
\end{equation}
where $\theta$ is the temperature, $\theta_0 = 293.15\,K$ is the reference ambient temperature, and $p_1$ to $p_5$ are design parameters. Selecting suitable values for $p_1$ to $p_5$ is a non-trivial task, as each parameter significantly influences the \ac{fgm}'s nonlinear field-grading behavior. For example, $p_1$ determines the baseline conductivity, while $p_2$ specifies the electric field strength where the \ac{fgm} transitions from baseline to nonlinear response. 
In this study, the parameters are initially set to $p_1 = 10^{-10}\,\text{S/m}$, $p_2 = 0.7\,$kV/m, $p_3 = 2.4$\,kV/m, $p_4 = 1864$ and $p_5 = 3713.59\,\+K$, with the field dependence at a fixed temperature illustrated in Fig.~\ref{fig:sigma_general}.

\begin{figure}[tb]	
	\centering
	\setlength{\fwidth}{0.45 \columnwidth}
%	\includegraphics[width=0.5\textwidth]{figs/ftsigma_RH.pdf}
	\input{figs/ftsigma_RH.tex}
	\caption{Nonlinear field- and temperature-dependent conductivity of the \ac{fgm}. The \ac{fgm} conductivity is modeled by the analytic function \eqref{Conductivity}.}
	\label{fig:sigma_general}
\end{figure}



